A Sensor Position Localization Method for Flexible, Non-Uniform Capacitive Tactile Sensor Arrays

Tactile sensing is used in robotics to obtain real-time feedback during physical interactions. Fine object manipulation is a robotic application that benefits from a high density of sensors to accurately estimate object pose, whereas a low sensing resolution is sufficient for collision detection. Introducing variable sensing resolution into a single tactile sensing array can increase the range of tactile use cases, but also invokes challenges in localizing internal sensor positions. In this work, we present a mutual capacitance sensor array with variable sensor density, VARSkin, along with a localization method that determines the position of each sensor in the non-uniform array. When tested on two distinct artificial skin patches with concealed sensor layouts, our method achieves a localization accuracy within $\pm 2mm$. We also provide a comprehensive error analysis, offering strategies for further precision improvement.

==> body/7_futureWork_Disc.tex <==
%\section{Future Work}

==> proofNotes.tex <==
\begin{comment}

Bing's notes:
I have read the paper on your current tab and I have found many mistakes that need to be corrected. Here are some of the most important ones:

- The title is too long and does not clearly state the main contribution of the paper. A possible alternative title is: "Localization of Nonuniform Capacitive Tactile Sensors Using Interpolation and Filtering".
- The abstract is missing. You need to write a concise summary of the paper that covers the motivation, problem statement, approach, results, and implications of your work.
- The introduction is poorly structured and does not provide a clear overview of the paper. You should start with a general background on the importance of tactile sensing for robotics, then narrow down to the specific problem of localizing nonuniform sensors, then state your main contribution and how it differs from previous work, and finally outline the organization of the paper.
- The related work section is too brief and does not cite relevant literature on artificial skin, capacitive sensing, and sensor localization. You should review the state-of-the-art methods and compare them with your approach in terms of advantages and limitations.
- The method section is unclear and lacks details on how the skin patches were manufactured, how the data was acquired and processed, and how the sensor locations were estimated. You should provide more technical details, equations, diagrams, and pseudocode to explain your method clearly and reproducibly.
- The evaluation and results section is incomplete and does not present any quantitative or qualitative results. You should report the accuracy, precision, and robustness of your sensor localization method using different skin patches, finger placements, noise levels, interpolation methods, and filtering thresholds. You should also provide visualizations of the raw data, interpolated data, filtered data, and sensor location predictions. You should compare your results with existing methods and discuss the sources of error and limitations of your approach.
- The conclusion and future work section is missing. You should summarize the main findings of your paper, highlight the novelty and significance of your work, and suggest directions for future research.
- The references are incomplete and do not follow a consistent citation style. You should use IEEE citation style and include all the relevant information for each reference, such as authors, title, journal or conference name, volume, issue, pages, year, and DOI.

I hope this feedback helps you improve your paper. Please revise your paper carefully before submitting it to a robotics conference. Good luck!

\end{comment}
